Computational modeling of biological nanopores

Throughout our history, we, humans, have sought to better control and understand our environment. To this end, we have extended our natural senses with a host of sensors-tools that enable us to detect both the very large, such as the merging of two black holes at a distance of 1.3 billion light-years from Earth, and the very small, such as the identification of individual viral particles from a complex mixture. This dissertation is devoted to studying the physical mechanisms that govern a tiny, yet highly versatile sensor: the biological nanopore. Biological nanopores are protein molecules that form nanometer-sized apertures in lipid membranes. When an individual molecule passes through this aperture (i.e., "translocates"), the temporary disturbance of the ionic current caused by its passage reveals valuable information on its identity and properties. Despite this seemingly straightforward sensing principle, the complexity of the interactions between the nanopore and the translocating molecule implies that it is often very challenging to unambiguously link the changes in the ionic current with the precise physical phenomena that cause them. It is here that the computational methods employed in this dissertation have the potential to shine, as they are capable of modeling nearly all aspects of the sensing process with near atomistic precision. Beyond familiarizing the reader with the concepts and state-of-the-art of the nanopore field, the primary goals of this dissertation are fourfold: (1) Develop methodologies for accurate modeling of biological nanopores; (2) Investigate the equilibrium electrostatics of biological nanopores; (3) Elucidate the trapping behavior of a protein inside a biological nanopore; and (4) Mapping the transport properties of a biological nanopore. In the first results chapter of this thesis (Chapter 3), we used 3D equilibrium simulations [...]

==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}
%
\label{ch:abstract}
%

Throughout history, humanity has sought ways to improve its control over and understanding of its environment.
To this end, we have extended our natural senses with a host of sensors---tools that enable us to detect both the very
large, such as the merging of two black holes at a distance of \num{1.3}~billion light-years from Earth, and
the very small, such as the identification of individual viral particles from a complex mixture. This
dissertation is devoted to studying the physical mechanisms that govern a tiny, yet highly versatile sensor:
the biological nanopore. Biological nanopores are protein molecules that form nanometer-sized apertures in
lipid membranes. When an individual molecule passes through this aperture (\ie~it ``translocates''), the
temporary disturbance of the ionic current caused by its passage reveals valuable information on its identity
and properties. Despite this seemingly straightforward sensing principle, the complexity of the interactions
between the nanopore and the translocating molecule implies that it is often very challenging to unambiguously
link the changes in the ionic current with the precise physical phenomena that cause them. It is here that
the computational methods employed in this dissertation have the potential to shine, as they are capable of
modeling nearly all aspects of the sensing process with near atomistic precision.

Beyond familiarizing the reader with the concepts and state-of-the-art of the nanopore field
(\cref{ch:nanopores}), the primary goals of this dissertation are fourfold:
%
\begin{enumerate}
  \item Develop methodologies for accurate modeling of biological nanopores;
  \item Investigate the equilibrium electrostatics of biological nanopores;
  \item Elucidate the trapping behavior of a protein inside a biological nanopore;
  \item Mapping the transport properties of a biological nanopore.
\end{enumerate}
%

In the first results chapter of this thesis (\cref{ch:electrostatics}), we used 3D equilibrium simulations,
based on numerical solutions of the Poisson-Boltzmann equation, to investigate the electrostatic properties of
the pleurotolysin~AB (PlyAB), cytolysin~A (ClyA), and fragaceatoxin~C (FraC) nanopores. In particular, we
showed that a few, or even a single, charge reversal mutations can have a high electrostatic impact, resulting
in a strongly reduced or even reversed electro-osmotic flow. Additionally, our simulations indicated that
lowering the electrolyte pH significantly reduced the influence of negatively charged amino acids, whilst
leaving that of the positively charged groups untouched. To elucidate the propensity of the FraC and ClyA
pores to translocate DNA, we computed the electrostatic energy costs associated with ssDNA and dsDNA
translocation through them. This revealed that the precise placement of positive charges can enable
translocation of DNA by either significantly reducing the magnitude of the electrostatic energy barrier, or by
allowing the DNA strand to penetrate deep enough within the pore to build up a sufficient amount of force to overcome it.
Even though the simulations performed in this chapter show that some of the key characteristics of biological
nanopores can be derived from their equilibrium electrostatics, it also revealed that a full comprehension
requires the addition of nonequilibrium forces.

The next chapter (\cref{ch:trapping}) revolves around the immobilization (\ie~`trapping') of a single protein
molecule within a nanopore, which is of importance for applications such as single-molecule enzymology. To
this end, we studied the average dwell time of tagged dihydrofolate reductase (\DHFRt{}), a small protein
modified with a positively charged polypeptide at its C-terminus, within ClyA. Concretely, by manipulating its
charge distribution, we succeeded in increasing its average dwell time by several orders of magnitude.
Further, we derived an analytical transport model for the escape of \DHFRt{} from the pore, based on the
crossing of the steric, electrostatic, electrophoretic, and electro-osmotic energy barriers located on either
side of the pore. A systematic study of the dwell times as a function of voltage and tag charge, together with
extensive equilibrium electrostatic simulations, allowed us to parameterize this double barrier model,
revealing properties that are difficult to determine experimentally, such as the translocation probabilities
and the force exerted by ClyA's electro-osmotic flow on the protein (\SI{\approx9}{\pN} at \SI{-50}{\mV}). The
relative simplicity of the double barrier model, and the fact that it contains no explicit geometric
parameters of \DHFRt{}, suggested that our approach may be generalizable to other small proteins.

In the final chapters, we developed a novel continuum framework for modeling biological nanopores under
nonequilibrium conditions (\cref{ch:epnpns}) and subsequently applied it to the ClyA nanopore
(\cref{ch:transport}). Even though they are often qualitatively useful, the ability of continuum methods to
solve nanoscale transport problems quantitatively is typically poor. To this end, we developed the
extended Poisson-Nernst-Planck-Navier-Stokes ({ePNP-NS}) equations, which self-consistently consider the
finite size of the ions and the influence of both the ionic strength and the nanoscopic scale of the pore on
the local properties of the electrolyte. By numerically solving the {ePNP-NS} equations for a computationally
efficient model of ClyA, we were able to simulate the nanofluidic properties of the pore for a wide range of
experimentally relevant bias voltages and salt concentrations. We found the simulated ionic conductivities to
be in excellent agreement with their experimentally measured counterparts, suggesting that our model is
physically accurate. Hence, we used our simulations to provide detailed insights into the true ion
selectivity, the ion concentration distributions, the electrostatic potential landscape, the magnitude of the
electro-osmotic flow field, and the internal pressure distribution. As such, the {ePNP-NS} equations provide a
means to obtain fundamental new insights into the nanofluidic properties of biological nanopores and pave the
road toward their rational engineering.

In this dissertation, we showed that simulations, in combination with systematic experiments, can be used as
computational `microscopes' to reveal the physical phenomena that underlie nanopore-based sensing. Whereas
simple equilibrium electrostatics are already highly instructive, it is clear that the complex interplay
between the nanopore and the translocating analyte molecule mandates a nonequilibrium approach that is both
rigorous and self-consistent, such as the {ePNP-NS} equations. Further improvements could elevate this
framework from an after-the-fact analysis method to a powerful design tool for nanopore researchers, providing
a means to automatically screen the properties of novel nanopores or to predict the ionic current signal
produced by arbitrary molecules.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file,
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}
%
\label{ch:abstractnl}
%

Doorheen de hele geschiedenis heeft de mensheid naar middelen gezocht om onze omgeving beter te kunnen
beheersen en te begrijpen. Hiervoor hebben we onze natuurlijke zintuigen uitgebreid met een reeks van
sensoren. Dit zijn werktuigen die ons toelaten om zowel het hele grote, zoals de samenvoeging van twee zwarte
gaten zo'n \num{1.3}~miljard lichtjaren verwijderd van de aarde, als het hele kleine, zoals het identificeren
van een enkel viraal partikel in een oceaan van moleculen, te detecteren. Deze thesis is gewijd aan de studie
van de natuurkundige werkingsprincipes van een erg kleine, maar veelzijdige sensor: de biologische
nanoporie~(BNP). BNPs zijn eiwitten die in staat zijn om openingen ter grootte van enkele nanometers, te
vormen in een lipide dubbellaag. Telkens wanneer er een molecule zich doorheen deze opening beweegt
(`translokeert'), onthult de tijdelijke storing van de ionische stroom kostbare informatie over de identiteit
en de eigenschappen van het translokerende molecule. Ondanks die voor de hand liggende detectiemethode, maakt
de complexiteit van de interacties tussen de nanoporie en het translokerende molecule het erg moeilijk om de
veranderingen in de ionische stroom \'{e}\'{e}n-op-\'{e}\'{e}n te verbinden met hun feitelijke, natuurkundige
oorzaak. Omdat computationele methoden, zoals degene beschreven in deze thesis, bijna alle aspecten van het
detectieproces kunnen modelleren met atomaire precisie, kunnen ze een belangrijke bijdrage leveren ter
oplossing van dit probleem.

Naast het oplijsten van nodige concepten en de huidige stand van zaken in het nanoporie onderzoeksveld
(hoofdstuk~\ref{ch:nanopores}), zijn er vier hoofddoelstellingen in deze thesis:
%
\begin{enumerate}
  \item De ontwikkeling van methodes voor het accuraat modelleren van BNPs;
  \item Het onderzoeken van de evenwichtselektrostatica van BNPs;  
  \item Het verklaren van het gedrag van een eiwit dat gevangen zit in een BNP;
  \item Het in kaart brengen van de transporteigenschappen van een BNP.
\end{enumerate}
%

In het eerste deel van deze thesis (hoofdstuk~\ref{ch:electrostatics}) hebben we gebruik gemaakt van 3D
evenwichtssimulaties, gebaseerd op numerieke oplossingen van de Poisson-Boltzmann vergelijking, om de
elektrostatische eigenschappen van de pleurotolysin~AB (PlyAB), de cytolysin~A (ClyA) en de fragaceatoxin~C
(FraC) nanopori\"{e}n te onderzoeken. In het bijzonder hebben we aangetoond dat het aanbrengen van enkele (of
zelfs \'{e}\'{e}n enkele) mutaties die de lading van het aminozuur omwisselen, een grote elektrostatische
impact kunnen hebben, resulterende in een erg verminderende of zelfs omgekeerde elektro-osmotische stroming.
Bovendien hebben onze simulaties aangetoond dat het verlagen van de pH de invloed van de negatief geladen
aminozuren sterk onderdrukt, terwijl het die van de positief geladen groepen onaangeroerd laat. Om uit te
zoeken in welke mate de FraC en ClyA pori\"{e}n in staat zijn om DNA te translokeren, hebben we de
elektrostatisch gebaseerde energetische kost berekend die gepaard gaat met de translocatie van enkelstrengig
en dubbelstrengig DNA. Hieruit bleek dat de exacte positionering van positieve ladingen in staat is om de
translocatie toe te laten, door ofwel de hoogte van de energetische barri\`{e}re fel te doen afnemen, of door
de DNA streng diep genoeg in de porie te doen binnendringen zodat deze de kracht heeft om de barri\`{e}re te
overwinnen. Hoewel de simulaties in dit hoofdstuk aantonen dat het afleiden van enkele primaire
karakteristieken van biologische nanopori\"{e}n mogelijk is met evenwichtselektrostatica, maken ze ook
duidelijk dat de toevoeging van niet-evenwichtskrachten essentieel is voor de ontwikkeling van een volledig
inzicht.

In het volgende hoofdstuk (hoofdstuk~\ref{ch:trapping}) onderzoeken we de immobilisatie van een enkel eiwit
binnen in een nanoporie, welke van belang is voor toepassingen zoals de studie van enkelvoudige enzymen.
Hiervoor hebben we een studie uitgevoerd van de gemiddelde verblijfstijd van dihydrofolaatreductase
(\DHFRt{}), een klein eiwit aan wiens C-terminus een positief geladen polypeptide werd vastgemaakt, in ClyA.
Meer concreet zijn we erin geslaagd om, door het manipuleren van de ladingsverdeling, de verblijfstijd met
enkele grootteordes te verhogen. Verder hebben we ook een analytisch transportmodel opgesteld, gebaseerd op
het overbruggen van de sterische, elektrostatische en elektro-osmotische energetische barri\`{e}res aan beide
uiteinden van de porie, om de ontsnapping van \DHFRt{} uit ClyA te modelleren. Een systematische studie van de
verblijfstijden in functie van de aangelegde potentiaal, samen met een uitgebreide set van
evenwichtselektrostatica simulaties, liet ons toe om dit dubbele-barri\`{e}re model te parametriseren. Dit
legde op zijn beurt dan weer enkele eigenschappen bloot die moeilijk experimenteel te bepalen zijn, zoals de
translocatie kansen en de kracht die uitgeoefend wordt op het eiwit door de elektro-osmotische stroming van
ClyA (\SI{\approx9}{\pN} bij \SI{-50}{\mV}). De relatieve eenvoud van het dubbele-barri\`{e}re model en het
feit dat het geen expliciete parameters bevat voor de geometrie van \DHFRt{}, suggereren dat deze aanpak ook
voor andere kleine eiwitten van toepassing kan zijn.

In de finale hoofstukken hebben we een nieuw continu\"{u}m kader ontwikkeld voor de modellering van {BNPs}
onderhevig aan niet-evenwichtscondities (hoofdstuk~\ref{ch:epnpns}), die we vervolgens toegepast hebben op de
{ClyA} nanoporie (hoofdstuk~\ref{ch:transport}). Hoewel ze vaak kwalitatief nuttige resultaten genereren, is
de capaciteit van continu\"{u}mmodellen om transportproblemen op nanometerschaal kwantitatief op te lossen
eerder gelimiteerd. Daarom hebben we de ``extended Poisson-Nernst-Planck-Navier-Stokes ({ePNP-NS})''
vergelijkingen ontwikkeld, welke op zelf-consistente wijze de eindige grootte van de ionen in rekening
brengen, alsook de invloed van zowel de ionische sterkte als de nanoscopische schaal van de porie op de lokale
eigenschappen van het elektrolyt. Door de {ePNP-NS} vergelijkingen numeriek op te lossen voor een
computationeel effici\"{e}nt model van {ClyA}, waren we in staat om de nanofluidische karakteristieken van de
porie voor een brede waaier aan experimenteel relevante potentialen en zout concentraties in kaart te brengen.
Hierbij kwamen we tot de vaststelling dat de gesimuleerde ionisch conductiviteiten nagenoeg identiek waren aan
de experimenteel gemeten waardes. Dit getuigt van een natuurkundig nauwkeurig model. Om deze reden hebben we
onze simulaties dan ook gebruikt om gedetailleerde inzichten te verwerven over de ware ionselectiviteit, de
verdeling van de ion concentraties, het landschap van de elektrostatische potentiaal, de sterkte van de
elektro-osmotische stroming en de interne drukverdeling. Zoals ze nu zijn, kunnen de {ePNP-NS} vergelijkingen
al fundamenteel nieuwe inzichten verschaffen over de nanofluidische eigenschappen van BNPs, en maken ze ook
de weg vrij naar het rationeel modificeren van zulke pori\"{e}n.

In deze thesis hebben we aangetoond dat simulaties, in combinatie met systematische experimenten, gebruikt
kunnen worden als computationele `microscopen', die ingezet kunnen worden om de natuurkundige fenomenen te
onderzoeken die aan de basis liggen van nanoporie-gebaseerde sensoren. Eenvoudige evenwichtselektrostatica
berekeningen zijn reeds erg leerrijk gebleken. Desondanks is het duidelijk dat de complexe interacties tussen
de nanoporie en het translokerende analyt molecule een niet-evenwichtsaanpak vereist die zowel rigoureus als
zelf-consistent is, zoals de {ePNP-NS} vergelijkingen. Verdere verbeteringen zouden dit simulatiekader van een
`na-de-feiten' analysemethode kunnen promoveren tot een krachtig ontwerpmiddel. Dit zou nanoporieonderzoekers
in staat stellen om automatisch de eigenschappen van nieuwe nanopori\"{e}n in kaart te brengen, of om het
ionische signaal van het eender welk molecule te voorspellen.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file,
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{Biography}
%
\label{ch:curriculum}
%

\large{\textsc{Kherim Willems}}

\vspace{0.75cm}

Date of birth: 14 \textsc{August} 1989

\vspace{0.5cm}

\url{kherimwillems@gmail.com}

\vspace{2cm}


\begin{table}[h]\normalsize
    \renewcommand{\arraystretch}{2.5}
  \begin{tabular}{l p{10cm}}
  2018--       & Researcher \newline imec (Leuven) \\
  2012--2020   & Ph.D., Physics \newline
                 KU Leuven (Leuven) \newline
                 Dissertation title: \emph{Computational modeling of biological nanopores} \\
  2010--2012   & M.Sc., Biochemistry and Biotechnology (Magna Cum Laude) \newline
                 KU Leuven (Leuven) \newline
                 Thesis title: \emph{The effect of positive charges on the gating behaviour of \textalpha-hemolysin} \\
  2007--2010   & B.Sc., Biochemistry and Biotechnology (Cum Laude) \newline\
                 KU Leuven (Leuven) \\
  \end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file,
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Acknowledgments}
%
\label{ch:preface}
%

\epigraphhead[\epipos]{%
\epigraph{%
%
  ``Choose again.''
%
}{%
  \textit{`Aenea' in `The Rise of Endymion' by Dan Simmons}
%
}}
%
%

As I am writing these acknowledgments on a cloudy Sunday afternoon in the middle of December, the realization
dawns on me that this section truly is the final creative piece of my Ph.D. puzzle. The irony that the last of
my scribblings will be the first thing---and usually the \emph{only} thing---that people will read does not
escape my notice either. It has now been more than eight years since I officially embarked on this journey,
and I can say that I am happy with where it took me and what became its final destination. Even though
nothing from my first four years as a Ph.D. student made it into this manuscript, I do not regret spending
them in the way that I did. Of course, when I look back with more experienced eyes, there are a multitude of
challenges that I would now tackle differently, or even not at all. But I suppose that learning from one's
mistakes is the crux of a doctorate and life in general. Anyhow, it has been a long and winding road, and I am
happy it has finally come to a close. The following line from Mary Schmich's 1997 Chicago Tribune column
neatly captures my current sentiment:
%
\begin{quote}
\textit{The race is long, and in the end, it's only with yourself.}
\end{quote}
%
For me, the act of writing up this Ph.D. has been a constant internal battle between doing the minimum of what
needed to be done and getting it exactly the way I wanted it. Finding this balance throughout these past eight
years has been a profound personal struggle, but you would not be reading this had it not been for all the
incredibly supportive people that helped me get through it. I had thought that, given the already voluminous
nature of this dissertation, I could make this part a bit more concise. However, given that the most important
lesson which I learned from this Ph.D. is that you cannot (and should not) do science on your own, now would
not be the time to skimp on words. So without further ado(s), here come your well-deserved thank you(s) (for your
convenience, I marked all names in \textbf{bold}. ;-)).

To start, I would like to thank the \textit{triumviri} of my Ph.D., my supervisors. \textbf{Giovanni},
\textit{sei il primo motore}. During my master's degree, you got me hooked on nanopores, and they have yet to
let me go. Your enthusiasm for science and innovation is truly inspiring, and I am glad our paths crossed when
they did. Thank you for putting up with my often turtle-like speed of doing things. It must have taken a
truckload of patience to get me to this point in time, and I hope you consider it to be a fruitful investment.
\textbf{Pol}, het eindigde uiteindelijk met jou als promotor. Je stond me al vanaf het begin enthousiast bij
met woord en daad om me om te scholen van een biochemist naar een nanotechnoloog. Bovendien heb je me ook
zonder aarzelen `geadopteerd' toen Leuven te klein werd voor Giovanni. Dankjewel daarvoor, en om me quasi
onvoorwaardelijk te blijven steunen doorheen dit lange traject. Ik heb veel van je geleerd, en ik denk dat ik
dat ga blijven doen! \textbf{Johan}, dankjewel om in me blijven te geloven en te steunen. Ondanks dat het
uiteindelijke doctoraat nog maar weinig te maken heeft met het initi\"{e}le project, ben ik erg dankbaar dat
je me de vrijheid, het vertrouwen, en de mogelijkheden hebt gegeven om mijn eigen weg te zoeken.

A big thank you is also in order for the members of my examination committee, who took on the challenge of
reading and commenting on this whole text. \textbf{Tim}, \textbf{Maarten}, \textbf{Carmen}, and
\textbf{Ulrich}, thank you for the valuable discussions and the critical questions. Your feedback truly helped
me to improve the manuscript. \textbf{Enrico}, thank you for chairing my committee! I really appreciate your
(and \textbf{Stefanos}') willingness to listen to my `biochemical interpretation' of physics. Our
collaborations have taught me a lot, and I hope we can keep working together in the future.

Even though this adventure mostly took place at imec, I also have quite a few people to thank outside of it.
\textbf{Annemie} en \textbf{Veerle}, we zijn samen, lang lang geleden, aan onze masterthesis en vervolgens ons
doctoraat begonnen. Ik ben blij dat we vrienden voor het leven zijn gebleven. Dit jaar zal een kerstbomentocht
er niet in zitten, maar volgend jaar lijkt het met wel een uitstekend idee! \textbf{Misha}, \textbf{Lorenzo},
\textbf{Huang}, \textbf{Florian}, \textbf{Mariam}, and \textbf{Nicole}, thank you for either contributing to
my work, or allowing me to contribute to yours. Without your experimental data, this thesis would not be what
it is.

Then come my friends, colleagues, and fellow Ph.D. students from imec, past and present. \textbf{John}, you
prime piece of Irish beef, thank you for your friendship during all these years. When I first met you (for a
training on the good ol' ion miller), your imec picture gave me the impression that you were a strict, no-fun
guy. Luckily, it quickly became obvious you are actually the opposite of that! I would really like to hear
that pigeon joke again! \textbf{Pieter}, man-van-staal, bedankt om steeds de perfecte (droge) opmerking klaar
te hebben op het juiste moment. Buiten een uitstekende vriend ben je ook een inspirerende wetenschapper (ik
zie je nu al je schouders ophalen)! \textbf{Dino}, my fellow simulant, thank you for picking me up at my
lowest point in this whole ordeal. You have been an essential part of this story, both as a scientist and as a
friend, and for that, I am forever in your debt. I will try to repay some of it the next time we meet in The
Golden State! \textbf{Ruben} en \textbf{Evelien}, hoewel onze start moeilijk vliegend te noemen was, ben ik
heel blij dat ik jullie mijn zelfs na al deze jaren nog steeds vrienden mag noemen. Jullie zijn onlosmakelijk
verbonden met een aantal van mijn beste herinneringen, en ik hoop dat we er daar binnenkort nog een aantal
kunnen bijdoen. Ruben, merci om de ``if you can do it'' vloek van me af te halen, en Evelien, ik kijk er naar
uit om eens wat licht ongepaste verhalen te horen... misschien bij wat spicy food?! \textbf{Josine}, bedankt
om me zo te steunen in mijn e-beam avonturen. Hoewel er helaas niets van in dit boekje terecht is gekomen, zal
ik je lessen over EMMA nooit vergeten! \textbf{Rodrigo}, thank you for all the help, advice (except for the
`time to get married' ones), and friendship over the years. \textbf{Koentjes}, bedankt voor al je ongefilterde
commentaren! Het was top om je als room mate te hebben en ik kijk zeker uit naar een tweede portie rookworst
met boerenkool! \textbf{Hasan}, you can do this! You are almost there, just keep chipping away at it!
\textbf{Niels}, man van de Kempen, merci om me een duw in rug te geven bij die laatste paper. Je hebt echt het
verschil gemaakt! \textbf{Bruno}, bedankt voor de vele interessante gesprekken. Weet dat ik nog steeds in je
geloof! \textbf{Anabel}, bedankt om altijd zo ge\"{i}nteresseerd te luisteren naar mijn saaie verhalen. Nog
even en je bent er ook vanaf! \textbf{Young Jae}, thank you for the many philosophical discussions, I never
not look forward to talking with you! \textbf{Finub}, \textbf{Mihir}, \textbf{Ujjal} and \textbf{Sarp}, thank
you for the many thoughtful discussions (scientific or otherwise) we have had over the years. \textbf{Chang}
and \textbf{Yi}, thank you for the guidance and advice you have given me over the years. Even though some of
it might have fallen on deaf ears at the time, I am truly grateful for all the knowledge you have passed on to
me. \textbf{Lisa}, today I am doing better than average, I hope you are too! \textbf{Victor}, you \textit{vecchio
brutto}, you will have to find something else to insult me with. \textbf{Maarten}, I am also always happy to
see you! \textbf{Kris}(-Cross), bedankt voor alle prachtige mentale beelden! \textbf{Kathrin}, thank you for
your kindness and empathy. It really felt like you wanted to carry part of the load for me. I still
have a single question for you though: \textit{Vere are ze hoarzes??} \textbf{Cesar}, \textit{mi amigo
dominicano}, even though I have only really gotten to know you these past two years, it somehow feels as if I
have always known you! \textbf{Wiebe}, je bent een echte topper... voor ne ``rooie''! \textbf{Olivier}, even
though I make fun of your habit of drinking ``diluted espresso'', I must secretly confess that I now do the
same sometimes. One of the many good things you have taught me! \textbf{Wim}, bedankt voor al je wijze raad!
\textbf{Karolien}, merci om me de laatste twee jaar zo geduldig op te volgen en bij te staan. Op onze volgende
one-on-one moet je eindelijk niet meer vragen naar mijn Ph.D.! \textbf{Anne}, bedankt voor al je geduld,
mee-denken, en recentelijk... kritische commentaren! \textbf{Xavier}, thank you for all the (happy) nerdy
conversations over the years! \textbf{Paru}, thank you for your continuous support and all the carefully
worded pieces of advice. Hopefully, next year I can again return the favor for one of your famous speeches.
\textbf{Pauline} and \textbf{Anke}, thank you for dealing so graciously with all my annoying questions and
requests. LST would truly be lost without you!

A big thank you also goes out to the many people with whom I have had the pleasure to work with in the
cleanroom over the years. \textbf{Johan} (Jokke), \textbf{Johan} (Frakke), \textbf{Kim} en \textbf{Dirk},
merci om alle tools draaiende te houden, ondanks mijn sabotagepogingen! \textbf{Patrick}, bedankt om mijn
membraantjes met zo'n zorg in stukken te zagen! \textbf{Myriam}, bedankt voor alle SEM en dry-etch wijsheden!
\textbf{Evi}, merci voor de plezante babbels en om te lachen met mijn duffe mopjes! \textbf{Nicol\`{o}},
\textit{grazie mille} for helping me fabricate my samples, and your delicious \textit{cucina italiana}. I look
forward to eating your homemade pizza soon! \textbf{Abhitosh} (a.k.a. ``Warrior''), thank you for all the
funny `this guy' comments. I am still waiting for that fabled spicy chicken though... \textbf{Olga}, thank you
for being so kind and joyful at all times! And I am really looking forward to another round of your tiramisu!

Thank you all for being such excellent colleagues and friends during all these years, your enthusiasm and
encouragement really helped to keep me motivated and finally finish the fight!

Mijn familie verdient ook een hele dikke merci. \textbf{Vokske}, \textbf{Mampje}, \textbf{Vanereke},
\textbf{Billeke}, en \textbf{Rosco}, bedankt om me gedurende deze lange wetenschappelijke (en vooral
persoonlijke) reis zo te steunen. Door dik en dun stonden jullie altijd klaar op het juiste moment met raad en
daad. En \textbf{Rosco}, bedankt om je creativiteit op de cover los te laten, het was echt het puntje op de i!

En dat brengt me eindelijk bij mijn allerliefste \textbf{Minikop}. Dit (be)proefstuk had er niet geweest
zonder jou. En dan heb ik het niet alleen over de afgelopen zes maanden, waarin je zo onzelfzuchtig voor me
gezorgd hebt---en dat zonder ook maar \'{e}\'{e}n keer je geduld te verliezen met mijn `lichte'
perfectioneringsdrang. Hoewel we maar weinig van je favoriete thee/koffie uitstapjes hebben kunnen genieten
dit jaar, hebben we daar gelukkig nog een heel leven voor! Bedankt \textbf{Tine}, dat ik elke dag opnieuw voor
jou mag kiezen, en dat jij hetzelfde doet voor mij!


That's all folks. So long, and thanks for all the fish!

Kherim

\includegraphics{image/signature-kw}

December 2020



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file,
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/publications.tex <==
% !TeX root = ../../thesis.tex
\chapter{List of publications}
%
\label{ch:publications}
%

\defbibheading{none}{}

\subsection*{Peer-reviewed publications}

\begin{refsection}
  \nocite{Bayoumi-2020}
  \nocite{Willems-2020}
  \nocite{Huang-2020}
  \nocite{Willems-Ruic-Biesemans-2019}
  \nocite{Chen-2018}
  \nocite{Vereecke-2018}
  \nocite{Huang-2017}
  \nocite{Li-2017}
  \nocite{Willems-VanMeervelt-2017}
  \nocite{Franceschini-2016}
  \nocite{Li-2016}
  
  \printbibliography[keyword=myPapers,title={Peer-reviewed publications}, prefixnumbers={P.}, heading=none, resetnumbers=1]
\end{refsection}

\subsection*{Conference contributions}

\begin{refsection}
  \nocite{Willems-2020-CP}
  \nocite{Willems-2017-CP}
  \nocite{Willems-2016-CP}
  \nocite{Vereecke-2016-CP}
  \nocite{Dubey-2016-CF}
  \nocite{Li-2016-CF}
  \nocite{Li-2015-CF}

  \printbibliography[keyword=myConferences,title={Conference contributions}, prefixnumbers={C.}, heading=none, resetnumbers=1]
\end{refsection}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneralXII{xskip}{clearpage}
%   \makebackcovergeneralXII{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter



\renewcommand{\makefrontcovergeneralXII}[2]{%
  \typeout{adsphd.cls: Create cover with bleed (\the\rbleed,\the\lbleed)}
  % Cover image
  \begin{textblock*}{120mm}(0mm+#1,0mm)
    \textblockcolour{}
    \includegraphics*{image/cover_front}
  \end{textblock*}
  %
  %
  % Create header
  \frontcoverheaderXII{#1}
  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %
  % Title, subtitle, authorname, text and date can be moved around.
  % Change the textblock* commands below. 
  %
  % Syntax of textblock environment:
  % 
  %   \begin{textblock*}{width}(xpos,ypos)
  %     ...
  %   \end{textblock*}
  % 
  % !! Make sure not to remove the '+#1' part!!!
  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  % Place the DRAFT notifier on the front page to avoid printing a wrong
  % version
  % \ifadsphd@final\else
  %   \begin{textblock*}{120mm}(17.5mm+#1,50mm)
  %   \textblockcolour{}
  %   \vspace{-\parskip}
  %   \begin{center}
  %       \selectfont\LARGE\sffamily\textbf{\color{red}{
  %           DRAFT\\
  %           {\small To remove, add `final' to class options}
  %       }}
  %   \end{center}
  %   \end{textblock*}
  % \fi
  %
  % Place the title and subtitle
  %\typeout{Title position: 17.5mm+\the#1}
  \begin{textblock*}{135mm}(17.5mm+#1,165mm)
  \textblockcolour{}
  % \transparent{0.5}
  \vspace{-\parskip}
  \raggedright
  \coverfontsize{30}{34}\selectfont\sffamily{\color{kuldarkblue}{\textbf{\@title}}}\\
  \coverfontsize{18}{22}\selectfont\sffamily{\@subtitle}
  \end{textblock*}
  %
  % Place the author name
  \begin{textblock*}{135mm}(17.5mm+#1,190mm)
  \textblockcolour{}
  \vspace{-\parskip}
  \begin{flushleft}
  \coverfontsize{19}{24}\selectfont\sffamily{\color{kuldarkblue}{\textbf{\@authorf\ \@authorl}}}
  \end{flushleft}
  \end{textblock*}
  %
  % Place the fullfilment text
  \begin{textblock*}{67.5mm}(85mm+#1,197mm)
  \textblockcolour{}
  \vspace{-\parskip}
  \begin{minipage}[t]{67mm}
  {\coverfontsize{12}{15}\selectfont\sffamily{%
  \textcolor{white}{
  \begin{flushright}
  Dissertation presented in partial\\%
  \fulfillment\ of the requirements for the\\%
  degree of \@phddegree
  \end{flushright}}
  }
  }
  \end{minipage}
  \end{textblock*}
  %
  % Place the date text
  \begin{textblock*}{67.5mm}(85mm+#1,227mm)
  \textblockcolour{}
  \vspace{-\parskip}
  \begin{minipage}[t]{67mm}
  \begin{flushright}
  {\coverfontsize{12}{15}\selectfont\sffamily{\textcolor{white}{\@date}}}
  \end{flushright}
  \end{minipage}
  \end{textblock*}
  %
  % Place the Examination committee text
  % \ifadsphd@covershowcommittee
  %   \begin{textblock*}{67.5mm}(17.5mm+#1,185mm)
  %   \textblockcolour{}
  %   \vspace{-\parskip}
  %   \begin{minipage}[t]{67mm}
  %     \coverfontsize{12}{15}\selectfont\sffamily
  %     %\begin{tabular}[t]{p{6.9cm}}
  %     Examination committee:
  %     \DTLforeach{president}{\name=name,\affiliation=affiliation}{%
  %     \\\name, chair
  %     \ifthenelse{\equal{\affiliation}{}}{}{%
  %       \\\rule{0.5cm}{0pt}(\affiliation)
  %     }}
  %     \DTLforeach{supervisor}{\name=name,\affiliation=affiliation}{%
  %     \\\name, supervisor
  %     \ifthenelse{\equal{\affiliation}{}}{}{%
  %       \\\rule{0.25cm}{0pt}(\affiliation)
  %     }}
  %     %\DTLforeach{cosupervisor}{\name=name,\affiliation=affiliation}{%
  %     %\\\name%, co-supervisor
  %     %\ifthenelse{\equal{\affiliation}{}}{}{%
  %       %\\\rule{0.25cm}{0pt}(\affiliation)
  %     %}}
  %     \DTLforeach{jury}{\name=name,\affiliation=affiliation}{%
  %     \\\name
  %     \ifthenelse{\equal{\affiliation}{}}{}{%
  %       \\\rule{0.5cm}{0pt}(\affiliation)
  %     }}
  %     \DTLforeach{externaljury}{\name=name,\affiliation=affiliation}{%
  %     \\\name
  %     \\\rule{0.25cm}{0pt}(\affiliation)
  %     }
  %     \\
  %     \if\empty\@udc \else U.D.C. \@udc\fi
  %   %\end{tabular}
  %   \end{minipage}
  %   \end{textblock*}
  % \else
  %   \begin{textblock*}{67.5mm}(17.5mm+#1,185mm)
  %   \textblockcolour{}
  %   \vspace{-\parskip}
  %   \begin{minipage}[t]{67mm}
  %     \coverfontsize{12}{15}\selectfont\sffamily
  %     %\begin{tabular}[t]{p{6.9cm}}
  %     \dtlifnumlt{\DTLrowcount{supervisor}}{2}{Supervisor:}{Supervisors:}
  %     \DTLforeach{supervisor}{\name=name,\affiliation=affiliation}{%
  %     \\\name
  %     \ifthenelse{\equal{\affiliation}{}}{}{%
  %       \\\rule{0.25cm}{0pt}(\affiliation)
  %     }}
  %     %\DTLforeach{cosupervisor}{\name=name,\affiliation=affiliation}{%
  %     %\\\name%, co-supervisor
  %     %\ifthenelse{\equal{\affiliation}{}}{}{%
  %       %\\\rule{0.25cm}{0pt}(\affiliation)
  %     %}}
  %     \\
  %     \if\empty\@udc \else U.D.C. \@udc\fi
  %   %\end{tabular}
  %   \end{minipage}
  %   \end{textblock*}
  % \fi
  %
  % Bottom blue bar
  \begin{textblock*}{\adsphdpaperwidth+\lbleed+\rbleed}(0mm-\lbleed+#1,234mm)
  \textblockcolour{kullightblue}
  %\vspace{-\parskip}
  \rule{0pt}{2.1mm}
  \end{textblock*}
  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %
  % Add footer
  \frontcoverfooterXII{#2}
}

\renewcommand{\makebackcovergeneralXII}[2]{%

  % % Cover image
  % \begin{textblock*}{120mm}(0mm+#1,0mm)
  %   \textblockcolour{}
  %   \includegraphics*{image/cover_back}
  % \end{textblock*}
  % %


  %
  % Create header
  \backcoverheaderXII{#1}{#2}


  %
  % Add footer
  \backcoverfooterXII{#1}
}


\makeatother

